The Structure of IR Luminous Galaxies at 100 Microns

We have observed twenty two galaxies at 100 microns with the Kuiper Airborne Observatory in order to determine the size of their FIR emitting regions. Most of these galaxies are luminous far-infrared sources, with L_FIR > 10^11 L_sun. This data constitutes the highest spatial resolution ever achieved on luminous galaxies in the far infrared. Our data includes direct measurements of the spatial structure of the sources, in which we look for departures from point source profiles. Additionally, comparison of our small beam 100 micron fluxes with the large beam IRAS fluxes shows how much flux falls beyond our detectors but within the IRAS beam. Several sources with point- like cores show evidence for such a net flux deficit. We clearly resolved six of these galaxies at 100 microns and have some evidence for extension in seven others. Those galaxies which we have resolved can have little of their 100 micron flux directly emitted by a point-like active galactic nucleus (AGN). Dust heated to ~40 K by recent bursts of non-nuclear star formation provides the best explanation for their extreme FIR luminosity. In a few cases, heating of an extended region by a compact central source is also a plausible option. Assuming the FIR emission we see is from dust, we also use the sizes we derive to find the dust temperatures and optical depths at 100 microns which we translate into an effective visual extinction through the galaxy. Our work shows that studies of the far infrared structure of luminous infrared galaxies is clearly within the capabilities of new generation far infrared instrumentation, such as SOFIA and SIRTF.

==> table1.tex <==
\begin{deluxetable}{lllclccl}
\tablecaption{Target Galaxies and Observation Log}
\tablecolumns{7}
\tablewidth{0pt}
\tablehead{
\colhead{Galaxy} &\colhead{R.A.} &\colhead{Dec.} &\colhead{Ref.} &
\colhead{Date} &\colhead{Rot.\tablenotemark{a}} &
\colhead{Calib.\tablenotemark{b}} \\ 
\colhead{} & \colhead{(1950)} &\colhead{(1950)} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} &
\colhead{} 
}
\startdata
MCG+02-04-025 &01:17:23.17    &$+$14:05:58.8       &2 & 06/01/94  &\phn0\phm{.0} &CEK\nl
III Zw 35     &01:41:47.90    &$+$16:51:06.3       &1 & 29/08/9   &\phn3.9       &IS\nl
UGC 02369     &02:51:15.9\phn &$+$14:46:03\phm{.0} &3 & 29/08/95  &\phn1.4       &IS\nl
NGC 1275      &03:16:29.5\phn &$+$41:19:52.2       &5 & 06/01/94  &18.5          &CEK\nl
VII Zw 31     &05:08:17.5\phn &$+$79:36:40\phm{.0} &8 & 12/08/94, 16/08/94 &15.2      &Pal.\nl
UGC 05101     &09:32:04.78    &$+$61:34:37.0       &3 & 06/01/94  &\phn0\phm{.0} &CEK\nl
NGC 3110      &10:01:32.0\phn &$-$06:13:56\phm{.0} &2 & 06/01/94  &\phn4.6       &CEK\nl
NGC 4151      &12:08:01.06    &$+$39:41:02       &9 & 06/01/94    &\phn6.0       &CEK\nl
UGC 08696     &13:42:51.71    &$+$56:08:14.3       &3 & 26/08/95  &\phn6.5       &IM\nl
NGC 6090      &16:10:24.58    &$+$52:35:05.4       &3 & 12/08/94, 16/08/94  &\phn9.7   &Pal.\nl
NGC 6286      &16:57:44.99    &$+$59:00:41.7       &3 & 16/08/94  &\phn7.2       &Pal.\nl
IRAS 1713+53  &17:13:14.14    &$+$53:13:49.3       &2 & 26/08/95, 29/08/95 &18.7      &IM,IS\nl
IRAS 1720-00  &17:20:47.87    &$-$00:14:15.9       &7 & 26/08/95  &\phn0\phm{.0} &IM\nl
UGC 10923     &17:36:23.6\phn &$+$86:46:38\phm{.0} &6 & 26/08/95, 29/08/95 &14.7      &IM,IS\nl
NGC 7469      &23:00:44.41    &$+$08:36:15.8       &3 & 16/08/94  &\phn0\phm{.0} &Pal.\nl
NGC 7541      &23:12:11.2\phn &$+$04:15:41\phm{.0} &2 & 12/08/94  &\phn4.2       &Pal.\nl
Zw 475.056    &23:13:33.1\phn &$+$25:17:01.6       &3 & 29/08/95  &\phn6.3       &IS\nl
NGC 7625      &23:18:00.0\phn &$+$16:57:07\phm{.0} &2 & 16/08/94  &\phn0\phm{.0} &Pal.\nl
NGC 7770      &23:48:49.9\phn &$+$19:49:13\phm{.0} &2 & 26/08/95  &\phn3.3       &IM\nl
NGC 7771      &23:48:52.1\phn &$+$19:50:01\phm{.0} &2 & 26/08/95  &\phn2.1       &IM\nl
Markarian 331 &23:48:54.1\tablenotemark{c} &
                               $+$20:18:28.8       &3 & 29/08/95  &\phn4.4       &IS\nl
UGC 12915     &23:59:08.3    &$+$23:13:00.0       &4 & 26/08/95\tablenotemark{d} &N &\phn3.9 &IM\nl

\tablenotetext{a}{Angle in degrees over which the array rotated during the observations.}
\tablenotetext{b}{Calibrator souce.  CEK: 1 Ceres, 52 Europa, and 97 Klotho average;
Pal: 2 Pallas; IM: 704 Interamnia and 56 Melete average; IS: 704 Interamnia and 386 Siegena average.}
\tablenotetext{c}{This is the pointing position. The CHYT position is actually 23:48:54.03.}
\tablenotetext{d}{UGC 12915 also was observed on 16 Aug. 1994, values given in the tables are for 
the Aug. 1995 observation (See Section 5.2.21)}

\tablerefs{
(1) Chapman et al. 1990; (2) Condon et al. 1990 (CHSS);
(3) Condon et al. 1991 (CHYT); (4) Condon et al. 1993;
(5) Harrington et al. 1983; (6) Kojoian et al. 1981; (7) Martin et al. 1989;
(8) Sage \& Solomon 1987; (9) Wilson \& Ulvestad 1982.}

\enddata
\end{deluxetable}


==> table2.tex <==
\begin{deluxetable}{lccccccc}
\tablecolumns{8}
\tablewidth{0pt}
\tablecaption{Distances, Luminosities, Radio Fluxes, and \textup{q}}
\tablehead{
\colhead{Galaxy} &
\colhead{Distance\tablenotemark{a}} &
\colhead{log $L_{FIR}$\tablenotemark{b}} &
\colhead{$S_{1.49 GHz}$} &
\colhead{Radio} &
\colhead{q} &
\colhead{Type} &
\colhead{Type} \\
\colhead{} &
\colhead{(Mpc)} &
\colhead{($L_{\sun}$)} &
\colhead{(mJy)} &
\colhead{Ref.} &
\colhead{} &
\colhead{} &
\colhead{Ref.}
}
\startdata
MCG+02-04-025 &123       &11.3  &\phn49.1    &3 &\phs$ 2.32$ &HII &9,13 \nl
III Zw 35     &108       &11.3  &\phn41.2    &3 &\phs$ 2.56$ &AGN &13 \nl
UGC 02369     &123       &11.3  &\phn50.0    &3 &\phs$ 2.32$ &HII &13 \nl
NGC 1275      &\phn 68   &10.7  &24000\tablenotemark{c} &5 &$- 0.44$ &AGN &12 \nl
VII Zw 31     &218       &11.6  &\phn41.6    &5 &\phs$ 2.28$ &HII &6  \nl
UGC 05101     &164       &11.8  &150.0       &3 &\phs$ 2.10$ &AGN &11,13 \nl
NGC 3110      &\phn 66   &10.9  &109.0       &3 &\phs$ 2.22$ &HII &13 \nl
NGC 4151      &\phn 17   &\phn9.5 & 332.0\tablenotemark{c} &2 &\phs$ 1.42$ &AGN &12 \nl
UGC 08696     &157       &11.9  &143.0       &3 &\phs$ 2.27$ &AGN &11,13 \nl
NGC 6090      &122       &11.2  &\phn46.4    &3 &\phs$ 2.27$ &HII &13 \nl
NGC 6286      &\phn 80   &11.0  &142.0       &3 &\phs$ 2.01$ &HII,AGN &9,13 \nl
IRAS 1713+53  &208       &11.6  &\phn25.8    &3 &\phs$ 2.51$ &HII &13 \nl
IRAS 1720-00  &174       &11.9  &102.0       &5 &\phs$ 2.33$ &HII &13 \nl
UGC 10923     &103       &11.0  &\phn48.2    &10 &\phs$ 2.19$ &\nodata &\nodata \nl
NGC 7469      &\phn 66   &11.3  &169.0       &3 &\phs$ 2.33$ &AGN &12,13 \nl
NGC 7541      &\phn 35   &10.7  &150.0       &3 &\phs$ 2.32$ &HII &7  \nl
Zw 475.056    &110       &11.2  &\phn33.6    &3 &\phs$ 2.53$ &AGN &13 \nl
NGC 7625      &\phn 23   &\phn9.9  &\phn42.0 &3 &\phs$ 2.50$ &HII &8  \nl
NGC 7770      &\phn 58   &10.2  &\phn16.5    &3 &\phs$ 2.37$ &HII &13 \nl
NGC 7771      &\phn 58   &11.0  &107.3       &3 &\phs$ 2.39$ &HII &13 \nl
Markarian 331 &\phn 72   &11.1  &\phn67.6    &3 &\phs$ 2.51$ &HII &13 \nl
UGC 12915     &\phn 61   &10.6  &\phn47.\phn &4 &\phs$ 2.26$ &HII &1  \nl

\tablenotetext{a}{This assumes $H_{0} = 75$ km s$^{-1}$ Mpc$^{-1}$ and is
corrected for Virgocentric infall.  Taken from refs (3) and (5) except for
NGC 4151 from Hunt \& Giovanardi (1992) and  UGC 10923 from Mazzaralla
et al. (1994).}
\tablenotetext{b}{Using distance in second column and FIR flux (see equation
3, section 5.1.2) appropriate
for the radio flux given in column 4} 
\tablenotetext{c}{variable}
\tablerefs{
(1) Bernl\"{o}hr 1993; 
(2) Condon 1987; (3) CHSS; (4) Condon et al. 1993; (5) Condon et al. 1996;
(6) Djorgovski et al. 1990; (7) Giuricin et al. 1994; (8) Li et al. 1993;
(9) Lonsdale et al. 1993; (10) Marx et al. 1994; (11) Sanders et al. 1988;
(12) Seyfert 1943, (13) Veilleux et al. 1996.}
\enddata
\end{deluxetable}


==> table3.tex <==
\begin{deluxetable}{lccccc}
\tablecaption{Asteroid Counts and Derived Responsivities}
\tablecolumns{6}
\tablewidth{0pt}
\tablehead{
\colhead{Asteroid} &\colhead{Predicted flux} &
\colhead{Counts} &\colhead{Counts} &
\colhead{Resp.\tablenotemark{a}} &
\colhead{Resp.\tablenotemark{b}} \\ 
\colhead{} &\colhead{(Jy)} &
\colhead{$\Sigma 1-10$} &\colhead{Detector 5} & 
\colhead{$\Sigma 1-10$} &
\colhead{Detector 5} 
} 
\startdata
\sidehead{01/06/1994}
1 Ceres   &$145\pm 14$  &$24375\pm 698$ &$11088\pm 216$ & & \nl
52 Europa &$39.4\pm 4$ &$7520\pm 562$  &$3319\pm 151$  &$196.3\pm 17  $ &$84.8\pm 6  $\nl
97 Klotho &$10.5\pm 1$ &$2168\pm 342$  &$858\pm 91$    & & \nl
\sidehead{08/12/94 and 08/16/94}
2 Pallas  &$74.0\pm 7$ &$8914\pm 961$  &$3829\pm 231$\tablenotemark{c} &
$125.5\pm 18  $ &$53.9\pm 6  $ \nl
\sidehead{08/26/95}
704 Interamnia &$43.9\pm 4$ &$7769\pm 625$  &$3889\pm 250$  &$239.5\pm 24  $ &$113.1\pm 10 $\nl
56 Melete      &$21.1\pm 2$ &$5970\pm 492$  &$2711\pm 190$\tablenotemark{c} \nl
\sidehead{08/29/1995}
704 Interamnia &$43.1\pm 4$ &$1067\pm 151$  &$452.7\pm 25.7$\tablenotemark{c} &
$30.4 \pm 3   $ &$13.0 \pm 1   $\nl
386 Siegena      &$19.5\pm 2$ &$656\pm 45  $  &$283.4\pm 12  $\tablenotemark{c} \nl

\tablenotetext{a}{Derived resposivity for $\Sigma 1-10$ detectors.
Corrected for filter response of the asteroids.
See section 4.1 for details.}
\tablenotetext{b}{Derived resposivity for detector 5 alone.
Corrected for filter response of the asteroids.
See section 4.1 for details.}
\tablenotetext{c}{Because of the mispointing mentioned in sections 3, and 4.1,
this value is derived from the two detectors (usually numbers 4 and 5)
with the highest number of counts. We fit a point source sized gaussian
to these two detectors and used the peak flux of the gaussian to estimate
the number of counts 5 would have had if we had pointed correctly.}

\enddata
\end{deluxetable}


==> table4.tex <==
\begin{deluxetable}{lccc}
\tablecaption{100 \micron\ Fluxes and Compactness}
\tablewidth{0pt}
\tablehead{
\colhead{Galaxy} &\colhead{100 \micron\ Flux from Det. 5} &
\colhead{100 \micron\ Flux from Sum} &
\colhead{100 \micron\ Flux from IRAS\tablenotemark{a}} \\
\colhead{} &
\colhead{(Jy)} &
\colhead{(Jy)} &
\colhead{(Jy)} 
}
\startdata
MCG+02-04-025 &$\phn 7.4\pm 1.0$ &$\phn 8.0 \pm 1.5$ &$\phn 9.6\pm 0.2$ \nl
III Zw 35     &    $15.0\pm 1.3$ &    $13.2 \pm 2.1$ &    $13.7\pm 0.2$ \nl
UGC 02369     &$    10.9\pm 1.1$ &$\phn 9.1 \pm 1.6$ &    $11.1\pm 0.2$ \nl
NGC 1275      &$\phn 6.0\pm 0.7$ &$\phn 7.5 \pm 1.5$ &$\phn 6.9\pm 0.4$ \nl
VII Zw 31     &$\phn 9.1\pm 1.7$ &$\phn 7.9 \pm 2.9$ &    $10.4\pm 0.1$ \nl
UGC 05101     &    $18.4\pm 2.0$ &    $19.2 \pm 3.4$ &    $21.2\pm 0.2$ \nl
NGC 3110      &    $15.1\pm 1.5$ &    $15.8 \pm 1.9$ &    $23.2\pm 0.1$ \nl
NGC 4151      &$\phn 3.7\pm 0.9$ &$\phn 4.1 \pm 1.9$ &$\phn 8.6\pm 0.4$ \nl
UGC 08696     &    $17.7\pm 2.1$ &    $17.3 \pm 2.9$ &    $22.4\pm 0.1$ \nl
NGC 6090      &$\phn 9.3\pm 1.9$ &$\phn 8.4 \pm 2.4$ &$\phn 9.3\pm 0.1$ \nl
NGC 6286      &    $20.7\pm 3.5$ &    $21.7 \pm 4.5$ &    $22.0\pm 0.1$ \nl
IRAS 1713+53  &$\phn 7.5\pm 1.6$ &$\phn 6.4 \pm 2.7$ &$\phn 8.4\pm 0.1$ \nl
IRAS 1720-00  &    $24.8\pm 3.2$ &    $19.4 \pm 4.0$ &    $37.6\pm 0.5$ \nl
UGC 10923     &$\phn 8.7\pm 1.0$ &$\phn 9.2 \pm 1.4$ &$10.2\phn \pm 1.\phn$ \nl
NGC 7469      &    $42.9\pm 5.3$ &    $40.5 \pm 6.9$ &    $34.9\pm 0.6$ \nl
NGC 7541      &    $36.0\pm 4.5$ &    $38.7 \pm 6.0$ &    $40.6\pm 0.1$ \nl
Zw 475.056    &    $11.5\pm 1.4$ &    $10.1 \pm 2.3$ &    $11.6\pm 0.1$ \nl
NGC 7625      &    $19.5\pm 3.2$ &    $19.7 \pm 3.1$ &    $17.2\pm 0.1$ \nl
NGC 7770      &$\phn 3.5\pm 1.7$ &$\phn 6.9 \pm 2.0$ & \nodata \nl
NGC 7771      &    $34.4\pm 3.4$ &    $37.6 \pm 4.5$ &    $37.4\pm 0.9$ \nl
Markarian 331 &    $24.2\pm 2.2$ &    $22.5 \pm 2.8$ &    $20.9\pm 0.2$ \nl
UGC 12915     &$\phn 9.7\pm 1.3$ &    $11.6 \pm 1.9$ &    $13.4\pm 0.2$ \nl

\tablenotetext{a}{IRAS fluxes are uncorrected for color from BGS, BGS2,
Edelson et al. 1987 (for NGC 4151), or Mazzarella et al.
1991 (for UGC 10923).}

\enddata
\end{deluxetable}


==> table5.tex <==
\begin{deluxetable}{lcccc}
\tablecolumns{5}
\tablewidth{0pt}
\tablecaption{Observed Galaxy Sizes}
\tablehead{
\colhead{Galaxy} &
\colhead{FWHM Gaussian\tablenotemark{a}} &
\colhead{$2 \times r_{o}$ from fit\tablenotemark{b}} &
\colhead{$2 \times r_{o}$ from fluxes\tablenotemark{c}} &
\colhead{Resolved?\tablenotemark{d}} \\
\colhead{} &
\colhead{($D_{g}$ in  \arcsec)} &
\colhead{($D_{e}$ in  \arcsec)} &
\colhead{(\arcsec)} &
\colhead{}
}
\startdata
MCG+02-04-025 &19.0     &11.0     &12.9        &      $\sim$Y \nl
III Zw 35     &\phn 8.2     &$<$12 &\nodata     &\phm{$\sim$}N \nl
UGC 02369     &$<$7  &$<$12 &\phn 8.4    &\phm{$\sim$}N \nl
NGC 1275      &30.0     &17.0     &10.1        &\phm{$\sim$}Y \nl
VII Zw 31     &$<$8  &$<$7 &10.0        &\phm{$\sim$}N \nl
UGC 05101     &20.6     &$<$12 &10.2        &      $\sim$Y \nl
NGC 3110      &23.7     &13.0     &22.6        &\phm{$\sim$}Y \nl
NGC 4151      &19.7     &$<$12 &24.7        &\phm{$\sim$}N \nl
UGC 08696     &\phn 3.0     &$<$12 &12.3 	     &      $\sim$Y \nl
NGC 6090      &12.5     &$<$12 &\phn 5.4    &\phm{$\sim$}N \nl
NGC 6286      &21.3     &12.0     &\phn 7.9    &      $\sim$Y \nl
IRAS 1713+53  &$<$8  &$<$12 &\phn 9.5    &\phm{$\sim$}N \nl
IRAS 1720-00  &$<$7  &$<$12 &16.0        &      $\sim$Y \nl
UGC 10923     &20.2     &11.0     &10.6        &\phm{$\sim$}Y \nl
NGC 7469      &14.0     &\phn 7.0 &\nodata     &      $\sim$Y \nl
NGC 7541      &23.0     &12.5     &\phn 9.7    &\phm{$\sim$}Y \nl
Zw 475.056    &\phn 4.5     &$<$12 &\phn 5.8    &\phm{$\sim$}N \nl
NGC 7625      &21.8     &13.0     &\nodata     &\phm{$\sim$}Y \nl
NGC 7770      &\nodata  &\nodata  &\nodata     &      $\sim$Y \nl
NGC 7771      &16.3     &$<$12 &\nodata     &\phm{$\sim$}N \nl
Markarian 331 &12.3     &$<$12 &\nodata     &\phm{$\sim$}N \nl
UGC 12915     &23.4     &14.0     &14.0        &\phm{$\sim$}Y \nl

\tablenotetext{a}{FWHM of emitting region from 1-D fit assuming the spatial distribution
of the flux is Gaussian and the convolving beam is a Gaussian of $\sigma = 15.6$\arcsec\
(FWHM = 26\arcsec). }
\tablenotetext{b}{Scale size of the galaxy with a model where $I = I_{o} e^{-r/r_{o}}$.
The 2-D galaxy model is convolved with a 2-D PSF and a 1-D fit is made by the calculated
flux in detectors 1-10 with the observed flux.}
\tablenotetext{c}{Scale size of the galaxy with a model where $I = I_{o} e^{-r/r_{o}}$.
Calculated from the detector 5 and IRAS fluxes (table 3) assuming a ``beam" of
36\arcsec\ for detector 5 and 4\arcmin\ for the IRAS flux.}
\tablenotetext{d}{Do we resolve the FIR emission from the galaxy?  Y means we do, $\sim$Y means
we have some evidence for extension, N means we see none. Note that objects for which the core is unresolved by comparison with the point source profile can still show evidence for extended emission.}

\tablecomments{Galaxies with
$D_{g} <  20$\arcsec and a $D_{e} < 6$\arcsec\ have unresolved cores (except for the high S/N
NGC 7469) and we do not claim the fits given in columns 2 and 3 represent the actual
size of the emitting region for the unresolved galaxes.  Galaxes with a Y or
$\sim$Y have values that truly represent the emitting region sizes to +15\% and
-20\%.  See section 4.2 for details.}

\enddata
\end{deluxetable}


==> table6.tex <==
\begin{deluxetable}{lccccrr}
\tablewidth{0pt}
\tablecaption{Temperatures and Optical Depths Derived Using Exponential Sizes} 
\tablehead{
\colhead{Galaxy} &
\colhead{60 \micron\tablenotemark{a}} &
\colhead{100 \micron\tablenotemark{a}} &
\colhead{$D_{e}$} &
\colhead{$T_{d}$\tablenotemark{b}} &
\colhead{$\tau_{100}$\tablenotemark{b}} &
\colhead{$A_{V}$\tablenotemark{c}} \\ 
\colhead{} &
\colhead{(Jy)} &
\colhead{(Jy)} &
\colhead{(\arcsec)} &
\colhead{(K)} &
\colhead{} &
\colhead{} 
}
\startdata
MCG+02-04-025 &\phn 8.9 &\phn 8.0 &\phm{$<$}11.0 &\phm{$\sim$}45   &$2.1 \times 10^{-3}$  &$1.6$       \nl
III Zw 35     &11.9     &13.8     &$<$12.0       &$\sim$40         &$>4.8 \times 10^{-3}$ &$>\phn 3.6$ \nl
UGC 02369     &\phn 7.9 &11.1     &$<$12.0       &$\sim$37         &$>5.3 \times 10^{-3}$ &$>\phn 3.9$ \nl
NGC 1275      &\phn 7.4 &\phn 6.9 &\phm{$<$}17.0 &\phm{$\sim$}44   &$8.4 \times 10^{-4}$  &$0.6$       \nl
VII Zw 31     &\phn 5.9 &10.4     &$<$\phn 7.0   &$\sim$34         &$>2.0 \times 10^{-2}$ &$>15.0$     \nl
UGC 05101     &13.0     &21.3     &$<$12.0       &$\sim$35         &$>1.3 \times 10^{-2}$ &$>\phn 9.5$ \nl
NGC 3110      &\phn 8.0 &15.8     &\phm{$<$}13.0 &\phm{$\sim$}32   &$1.1 \times 10^{-2}$  &$8.3$       \nl
NGC 4151      &\phn 3.2 &\phn 4.1 &$<$12.0       &$\sim$38         &$>1.7 \times 10^{-3}$ &$>\phn 1.3$ \nl
UGC 08696     &22.1     &22.4     &$<$12.0       &$\sim$42         &$>6.3 \times 10^{-3}$ &$>\phn 4.7$ \nl
NGC 6090      &\phn 6.3 &\phn 9.3 &$<$12.0       &$\sim$36         &$>4.8 \times 10^{-3}$ &$>\phn 3.6$ \nl
NGC 6286      &\phn 8.4 &21.7     &\phm{$<$}12.0 &\phm{$\sim$}30   &$2.6 \times 10^{-2}$  &$20.0$      \nl
IRAS 1713+53  &\phn 6.4 &\phn 8.4 &$<$12.0       &$\sim$37         &$>3.6 \times 10^{-3}$ &$>\phn 2.7$ \nl
IRAS 1720-00  &17.9     &19.4     &$<$12.0       &$\sim$42         &$>6.0 \times 10^{-3}$ &$>4.2$     \nl
UGC 10923     &\phn 4.7 &10.2     &\phm{$<$}11.0 &\phm{$\sim$}31   &$1.1 \times 10^{-2}$  &$ 8.3$      \nl
NGC 7469      &27.7     &34.9     &\phm{$<$}\phn7.0 &\phm{$\sim$}39   &$4.0 \times 10^{-2}$ &$30.0$    \nl
NGC 7541      &20.6     &40.6     &\phm{$<$}12.5 &\phm{$\sim$}33   &$3.0 \times 10^{-2}$  &$23.0$      \nl
Zw 475.056    &\phn 8.8 &11.6     &$<$12.0       &$\sim$37         &$>5.0 \times 10^{-3}$ &$>\phn 3.8$ \nl
NGC 7625      &\phn 8.6 &17.2     &\phm{$<$}13.0 &\phm{$\sim$}32   &$1.2 \times 10^{-2}$  &$9.0$       \nl
NGC 7770      &\phn 2.6 &\phn 4.8 &$<$12.0       &$\sim$33         &\nodata               &\nodata     \nl
NGC 7771      &17.8     &32.6     &$<$12.0       &$\sim$33         &$>2.3 \times 10^{-2}$ &$>17.0$     \nl
Markarian 331 &17.3     &20.9     &$<$12.0       &$\sim$39         &$>7.7 \times 10^{-3}$ &$>\phn 5.8$ \nl
UGC 12915     &\phn 5.4 &11.6     &\phm{$<$}14.0 &\phm{$\sim$}31   &$7.7 \times 10^{-3}$  &$5.8$       \nl

\tablenotetext{a}{Fluxes quoted are from IRAS unless the 100 \micron\ IRAS flux is
beyond our errors or a companion galaxy complicates the system.
See section 5.2 to deterimine the source of the
flux we used in any particular galaxy.  Usually if we did not use the IRAS point we
used our 100 \micron\ point and
a 60 \micron\ point scaled so that the ratio of 60 and 100 \micron\ fluxes is the same
as for IRAS.}
\tablenotetext{b}{These parameters derived from simple single slab model with an emitting region
area = $\pi(\onehalf D_{e})^{2}$ and n = 1.5 where dust emissivity, $Q \propto \lambda^{-n}$.}
\tablenotetext{c}{Using $A_{V} / \tau_{100} = 750$ (Makinen et al. 1985).}

\enddata
\end{deluxetable}


==> table7.tex <==
\begin{deluxetable}{lccccrr}
\tablewidth{0pt}
\tablecaption{Temperatures and Optical Depths Derived Using Gaussian Sizes}
\tablehead{
\colhead{Galaxy} &
\colhead{60 \micron\tablenotemark{a}} &
\colhead{100 \micron\tablenotemark{a}} &
\colhead{$D_{g}$} &
\colhead{$T_{d}$\tablenotemark{b}} &
\colhead{$\tau_{100}$\tablenotemark{b}} &
\colhead{$A_{V}$\tablenotemark{c}} \\
\colhead{} &
\colhead{(Jy)} &
\colhead{(Jy)} &
\colhead{(\arcsec)} &
\colhead{(K)} &
\colhead{} &
\colhead{}
}
\startdata
MCG+02-04-025 &\phn 8.9 &\phn 8.0 &19.0 &45   &$7.2 \times 10^{-4}$ &0.5 \nl
NGC 1275      &\phn 7.4 &\phn 6.9 &30.0 &44   &$2.7 \times 10^{-4}$ &0.2 \nl
NGC 3110      &\phn 8.0 &15.8     &23.7 &32   &$3.3 \times 10^{-3}$ &2.5 \nl
NGC 6286      &\phn 8.4 &21.7     &21.3 &30   &$8.4 \times 10^{-3}$ &6.3 \nl
UGC 10923     &\phn 4.7 &10.2     &20.2 &31   &$3.4 \times 10^{-3}$ &2.6 \nl
NGC 7469      &27.7     &34.9     &14.0 &38   &$1.0 \times 10^{-2}$ &7.5 \nl
NGC 7541      &20.6     &40.6     &23.0 &32   &$8.8 \times 10^{-3}$ &6.6 \nl
NGC 7625      &\phn 8.6 &17.2     &21.8 &32   &$4.3 \times 10^{-3}$ &3.2 \nl
UGC 12915     &\phn 5.4 &11.6     &23.4 &31   &$2.8 \times 10^{-3}$ &2.1 \nl

\tablenotetext{a}{Fluxes quoted are from IRAS unless the 100 \micron\ IRAS flux is
beyond our errors.  See section 5.2 to deterimine the source of the
flux we used in any particular galaxy.  Usually if we did not use the IRAS point we
used our 100 \micron\ point and
a 60 \micron\ point scaled so that the ratio of 60 and 100 \micron\ fluxes is the same
as for IRAS.}
\tablenotetext{b}{These parameters are derived from a simple single slab model with an
emitting region \mbox{area = $\pi(\onehalf FWHM)^{2}$} and n = 1.5 where dust emissivity,
$Q \propto \lambda^{-n}$.}
\tablenotetext{c}{Using $A_{V} / \tau_{100} = 750$ (Makinen et al. 1985).}

\enddata
\end{deluxetable}


==> table8.tex <==
%\documentstyle[apjpt4]{article}
%\begin{document}
\begin{deluxetable}{cccccrrr}
%\tablenum{7}
\tablewidth{352.15288pt}
%\tablewidth{0pt}
\tablecolumns{8}
\tablecaption{Temperatures, Optical Depths, and Emissivity Exponents 
Derived from \mbox{60 $\mu$\textup{m},} 100 $\mu$\textup{m}, and Longer Wavelengths.}
\tablehead{
\colhead{$\lambda$} &
\colhead{Flux} &
\colhead{Ref.} &
\colhead{$D_{e}$} &
\colhead{$T_{d}$\tablenotemark{a}} &
\colhead{$\tau_{100}$\tablenotemark{a}} &
\colhead{$A_{V}$\tablenotemark{b}} &
\colhead{n\tablenotemark{a}} \\
\colhead{(\micron)} &
\colhead{(Jy)} &
\colhead{} &
\colhead{(\arcsec)} &
\colhead{(K)} &
\colhead{} &
\colhead{} &
\colhead{} 
}
\startdata
\sidehead{UGC 05101}
\phm{10}60 &\phm{$<$}13.0\phm{00} &2 &$<12.0$ &$\sim 35  $ &
$>1.3 \times 10^{-2}$ &$>8.5$ &$\sim 1.50$ \nl
\phm{1}100 &\phm{$<$}21.3\phm{00} &2 & & & & & \nl
\phm{1}350 &\phn $<$2.644         &7 & & & & & \nl
\phm{1}450 &\phn\phm{$<$}1.433    &7 & & & & & \nl
\phm{1}800 &\phn\phm{$<$}0.143    &7 & & & & & \nl
1100       &\phn\phm{$<$}0.068    &7 & & & & & \nl
1250       &\phn $<$0.036         &3 & & & & & \nl
\sidehead{NGC 3110}
\phm{10}60 &\phn\phm{$<$}8.0\tablenotemark{c}\phm{00} &1,2 &$\phm{<}13.0$ &
$\phm{\sim}32  $ &$>1.1 \times 10^{-2}$ &$8.3$ &$1.55$ \nl
\phm{1}100 &\phm{$<$}15.8\phm{00}    &1 & & & & & \nl
1250       &\phn\phm{$<$}0.033\tablenotemark{c} &1,3 & & & & & \nl
\sidehead{UGC 08696}
\phm{10}60 &\phm{$<$}22.1\phm{00} &2 &$<12.0$ &$\sim 42  $ &
$>6.4 \times 10^{-3}$ &$> 4.8$ &$\sim 1.51$ \nl
\phm{1}100 &\phm{$<$}22.4\phm{00} &2 & & & & & \nl
\phm{1}350 &\phn\phm{$<$}1.004    &7 & & & & & \nl
\phm{1}450 &\phn\phm{$<$}0.707    &7 & & & & & \nl
\phm{1}800 &\phn\phm{$<$}0.084    &7 & & & & & \nl
1100       &\phn\phm{$<$}0.051    &7 & & & & & \nl
1250       &\phn $<$0.063         &7 & & & & & \nl
1300       &\phn\phm{$<$}0.020    &5 & & & & & \nl
\sidehead{NGC 6090}
\phm{10}60 &\phn\phm{$<$}6.3\phm{00} &2 &$<12.0$ &$\sim 31  $ &
$>8.9 \times 10^{-3}$ &$>6.7$ &$\sim 2.28$ \nl
\phm{1}100 &\phn\phm{$<$}9.3\phm{00} &2 & & & & & \nl
1300       &\phn\phm{$<$}0.003       &4 & & & & & \nl
\sidehead{NGC 6286}
\phm{10}60 &\phn\phm{$<$}8.4\phm{00} &8 &$\phm{<}12.0$ &$\phm{\sim}29  $ &
$3.2 \times 10^{-2}$ &$24.0$ &$1.77$ \nl
\phm{1}100 &\phm{$<$}21.7\phm{00}    &1 & & & & & \nl
1250       &\phn\phm{$<$}0.040       &3 & & & & & \nl
\sidehead{UGC 10923}
\phm{10}60 &\phn\phm{$<$}4.7\phm{00} &6 &$\phm{<}11.0$ &$\sim 28   $ &
$>1.9 \times 10^{-2}$ &$>14.5$ &$>2.20$ \nl
\phm{1}100 &\phm{$<$}10.2\phm{00}    &6 & & & & & \nl
1300       &\phn$<$0.006             &4 & & & & & \tablebreak
\sidehead{NGC 7469}
\phm{10}60 &\phm{$<$}27.7\phm{00} &2 &$\phm{<}\phn7.0$ &$\sim 37  $ &
$>4.6 \times 10^{-2}$ &$>35.0$ &$>1.69$ \nl
\phm{1}100 &\phm{$<$}34.9\phm{00}    &2 & & & & & \nl
1250       &\phn$<$0.033             &3 & & & & & \nl
\sidehead{NGC 7541}
\phm{10}60 &\phm{$<$}20.6\phm{00} &2 &$\phm{<}12.5$ &$\phm{\sim}32  $ &
$3.4 \times 10^{-2}$ &$26.0$ &$1.67$ \nl
\phm{1}100 &\phm{$<$}40.6\phm{00}    &2 & & & & & \nl
1250       &\phn\phm{$<$}0.067       &3 & & & & & \nl
\sidehead{NGC 7771}
\phm{10}60 &\phm{$<$}17.8\tablenotemark{d}\phm{00} &1,2 &$<12.0$ &$\sim 33  $ &
$>2.3 \times 10^{-2}$ &$>17.0$ &$\sim 1.49$ \nl
\phm{1}100 &\phm{$<$}32.6\tablenotemark{d}\phm{00} &1,2 & & & & & \nl
1250       &\phn\phm{$<$}0.070       &3 & & & & & \nl
\sidehead{Markarian 331}
\phm{10}60 &\phm{$<$}17.3\phm{00} &2 &$<12.0$ &$\sim 35  $ &
$>1.5 \times 10^{-2}$ &$>8.6$ &$>2.01$ \nl
\phm{1}100 &\phm{$<$}20.9\phm{00}    &2 & & & & & \nl
1300       &\phn$<$0.009             &4 & & & & & \nl
\tablenotetext{a}{These parameters are derived from a simple single slab model with an
emitting region \mbox{area = $\pi(\onehalf FWHM)^{2}$} and $Q \propto \lambda^{-n}$.}
\tablenotetext{b}{Using $A_{V} / \tau_{100} = 750$ (Makinen et al. 1985).}
\tablenotetext{c}{We use our ``small beam" 100 \micron\ flux for NGC 3110 so the
60 and 1250 \micron\ points quoted here are scaled so that the ratio of each to
the 100 \micron\ flux remains the same as in was for the large beam (IRAS) flux.}
\tablenotetext{d}{The IRAS flux is a combination of NGC 7770 and 7771.  The value
we quote here is an estimate for NGC 7771 only using the BGS flux as a starting
point.  See section 5.2.19 for details.}
\tablerefs{
(1) This Paper; (2) BGS; (3) Carico et al. 1992; (4) Chini et al. 1992;
(5) Kr\"{u}gel et al. 1988; (6) Mazzarella et al. 1991; (7) Rigopoulou et al. 1996a;
(8) Surace et al. 1993.} 
\enddata
\end{deluxetable}
%\end{document}

